Higher-Order Function Networks for Learning Composable 3D Object Representations

We present a new approach to 3D object representation where a neural network encodes the geometry of an object directly into the weights and biases of a second 'mapping' network. This mapping network can be used to reconstruct an object by applying its encoded transformation to points randomly sampled from a simple geometric space, such as the unit sphere. We study the effectiveness of our method through various experiments on subsets of the ShapeNet dataset. We find that the proposed approach can reconstruct encoded objects with accuracy equal to or exceeding state-of-the-art methods with orders of magnitude fewer parameters. Our smallest mapping network has only about 7000 parameters and shows reconstruction quality on par with state-of-the-art object decoder architectures with millions of parameters. Further experiments on feature mixing through the composition of learned functions show that the encoding captures a meaningful subspace of objects.

==> old_section3point2.tex <==

\subsection{Comparing with LVC Methods}
\label{sec:comparing}
We compare our \FuncName{} approach with LVC architectures such as DeepSDF~\citep{park2019deepsdf} and FoldingNet~\citep{yang2018foldingnet}. These architectures control the output of the decoder through the concatenation of a latent `codeword' vector with each input $\vec{x_i} \in \set{X}$. We consider the case in which the latent vector is only concatenated with inputs in the first layer of the decoder network $\Dec{}$, which we assume to be an MLP. We are interested in analyzing the manner in which the network output with respect to $\vec{x_i}$ may be modulated by varying $\vec{z}$.

If the vector $\vec{a_i}$ contains the pre-activations of the first layer of $\Dec{}$ given an input point $\vec{x_i}$, we have
\begin{equation*}
    \vec{a_i} = W^\vec{x}\vec{x_i} + W^\vec{z}\vec{z} + \vec{b}
\end{equation*}

where $W^\vec{x}$, $W^\vec{z}$, and $\vec{b}$ are fixed, and only $\vec{z}$ is a function of $I$. If we absorb the parameters $W^\vec{z}$ and $\vec{b}$ into $\phi$ (as $W^\vec{z}$ and $\vec{b}$ are fixed for all $\vec{x_i}$), we can define a new, equivalent latent representation $\vec{b}^*=W^\vec{z}\vec{z} + \vec{b}=h(I)$ for some $h$. This gives
\begin{equation*}
    \vec{a_i} = W^\vec{x}\vec{x_i} + h(I)
\end{equation*}

Thus the LVC approach is equivalent to estimating a \textit{fixed subset} of the parameters $\theta$ of the decoder $\Dec{}$ on a per-sample basis (the bias). From this perspective, \method{} is an intuitive generalization: rather than estimating just the bias, we allow our encoder to modulate all of the parameters in the decoder $\Dec{}$ on a per-sample basis.

Having demonstrated HOF as a generalization of existing contextual mapping methods,
in the next section, we present a novel application of contextual mapping that leverages the compositionality of the estimated mapping functions to aggregate features of multiple objects or multiple viewpoints of the same object. %Results of a quantitative evaluation of this approach can be found in Figure~\ref{fig:performance_multiview}.

%some (potentially arbitrarily chosen) subset of $\theta$ on a per-sample basis, we might allow our encoder to \textit{learn} which parameters in the decoder $\Dec{}$ should be fixed, and which should vary per-sample. 

% The observation that LVC methods reduce the codeword to an additive bias is formalized in Proposition~\ref{lem:codeword-is-bias}.
% \label{sec:proof}
% \begin{proposition}
% \label{lem:codeword-is-bias}
% If $\Dec{}$ is an MLP with no skip connections computing outputs as $\Dec{}(\vec{x};\vec{z})=\Dec{}(\begin{bmatrix}\vec{z}\\\vec{x}\end{bmatrix})$, $\vec{z}$ acts as a bias $\vec{b}$ to the first layer pre-activations computed independently for each sample.
% \end{proposition}

% Further, we note that if $\vec{b}$ is lower dimensional than $\vec{z}$, there exists infinite $\vec{z}^*$ that satisfy $W^\vec{z}\vec{z}^* = W^\vec{z}\vec{z} + \vec{b}$. Thus, if the latent vector $\vec{z}$ is higher dimensional than the activations in the first layer of $\Dec{}$, we see a degeneracy; the additional expressiveness from the higher dimensional $\vec{z}$ is in some sense wasted.

% The \method{} regime follows as a generalization of LVC contextual mapping methods when $|\vec{b}| < |\theta|$, that is, there are other parameters of the mapping function $\Dec{}$ other than biases in the first layer. We call this assumption that $|\vec{b}| < |\theta|$, where the inequality is strict, our \textbf{non-degeneracy assumption} with respect to the architecture of $\Dec{}$. Given this assumption, we make a final observation about the expressiveness of the \method{} regime in comparison to the LVC regime.

% We consider an encoder network $\Enc$ whose final layer is fully-connected and a fixed mapping network architecture $A_\text{Map}$. We define $\mathcal{H}$ and $\mathcal{L}$ as the spaces of all \FuncName{} parameters for architecture $A_\text{Map}$ that can be estimated from an input image $I$ by the \method{} and LVC regimes, respectively, by $\Enc$. Our claim is stated in Theorem~\ref{thm:codeword-bad}.
% \begin{theorem}
% \label{thm:codeword-bad}
% $\mathcal{L} \subseteq \mathcal{H}$. If the network architecture satisfies our non-degeneracy assumption, $\mathcal{L} \subset \mathcal{H}$.
% \end{theorem}

% \newcommand{\memA}{\gamma}
% \newcommand{\memB}{\beta}
% \begin{proof}
% $\mathcal{L} \subseteq \mathcal{H}$ follows from Proposition~\ref{lem:codeword-is-bias} because \method{} can compute all parameters in $\Dec{}$ given an input $I$ while LVC can only compute the first layer biases. To show that the subset is strict, we define two sets of parameters $\memA$ and $\memB$ in $\mathcal{H}$ such that $\memA = \begin{bmatrix}\vec{b}\\\vec{p}\end{bmatrix}$ and $\memB = \begin{bmatrix}\vec{b}\\\vec{q}\end{bmatrix}$. $|\vec{p}| = |\vec{q}| > 0$ by our non-degeneracy assumption. If $\vec{p} \neq \vec{q}$, $\memA$ and $\memB$ cannot both be in $\mathcal{L}$ because under LVC, parameters in the mapping network other than the first layer bias are fixed.
% \end{proof}



==> theorem.tex <==
\subsection{Comparing with LVC Methods}
\label{sec:comparing}
We compare our \FuncName{} approach with LVC architectures such as DeepSDF~\citep{park2019deepsdf} and FoldingNet~\citep{yang2018foldingnet}. These architectures control the output of the decoder through the concatenation of a latent `codeword' vector with each input $\vec{x} \in \set{X}$. For example, $\vec{x}$ can be the coordinates where a value such as occupancy or signed distance will be  estimated by the network. Our main claim is that HOF architectures are more general than LVC architectures. 


To formalize this claim, consider the set of LVC methods which take input (in our case an image)~$I$ and generate a codeword $c(I)$ based on the image. The decoder is assumed to be an MLP which takes  $\vec{x}$ concatenated with $c(I)$ as its input.
Once learned, the weights of the MLP are fixed. 
We allow concatenation to happen at multiple layers as in~\cite{park2019deepsdf}. Let  $\mathcal{L}$ be the space of all such functions represented by this LVC architecture. We define the complexity of an LVC-based function $l \in \mathcal{L}$ as the total number of network parameters in $l$ plus the length of the codeword. $\mathcal{L}_n$ denotes the set of LVC architectures whose complexity is at most $n$.

For the HOF architecture, we consider a similar coding scheme. However, we let the encoder generate an arbitrary function $f_I$ (the decoder itself) conditioned on the input $I$. Once generated, $f_I$ takes vector $\vec{x}$ as input and generates the value to be estimated directly as $f_I(\vec{x})$. The complexity of the HOF architecture is given by the total number of parameters of the encoder and its output, the decoder.


Our key insight is that the LVC approach is equivalent to estimating a \textit{fixed subset} of the parameters of the decoder on a per-sample basis (the bias). From this perspective, \method{} is an intuitive generalization: rather than estimating just the bias, we allow our encoder to modulate all of the parameters in the decoder on a per-sample basis. This insight is formalized in the following theorem which is proven in  Appendix~\ref{sec:proof_appendix}.

\begin{theorem}
\label{thm:codeword-bad}
Let  $\mathcal{L}_n$ and $\mathcal{H}_n$ be the sets of all functions with complexity at most $n$  represented by the LVC and HOF architectures respectively. 
$\mathcal{L}_n \subset \mathcal{H}_n$.
\end{theorem}



\newcommand{\memA}{\gamma}
\newcommand{\memB}{\beta}
\begin{proof}
First we show that $\mathcal{L}_n \subseteq \mathcal{H}_n$. To do this, consider $l \in \mathcal{L}_n$. We will show that there exists an $h \in \mathcal{H}$ which computes the same mapping as $l$.

Consider the decoder of $l$. Let $\vec{x_i}$ be an input vector which is concatenated with the codeword $\vec{z} = c(I)$ and input to the layer $i$ of the decoder whose pre-activations are given by the vector $\vec{a_i}$. Since the decoder is an MLP, we have

\begin{equation*}
    \vec{a_i} = W^\vec{x}\vec{x_i} + W^\vec{z}\vec{z} + \vec{b}
\end{equation*}

where $W^\vec{x}$, $W^\vec{z}$, and $\vec{b}$ are fixed, and only $\vec{z}$ is a function of $I$. Since $W^\vec{z}$ and $\vec{b}$ are fixed for all $\vec{x_i}$, we can define a new, equivalent latent representation $\vec{b}^\prime(I)=W^\vec{z}\vec{z} + \vec{b}$. This gives
\begin{equation*}
    \vec{a_i} = W^\vec{x}\vec{x_i} + b^\prime(I)
\end{equation*}


We will now show that there exists an $h \in \mathcal{H}$ which computes the same mapping as $l$.
 The decoder of $h$ is also an MLP whose weights at layer $i$ are given by $W^\vec{x}$ and $b^\prime(I)$. The encoder will output these weights, and therefore $h$ computes exactly the same values as $l$. It can be verified that the complexity of $h$ is at most the complexity of $l$ which is at most $n$.

To see that $\mathcal{L}$ is a strict subset of $\mathcal{H}$, consider the same function $l$ as above. Note that once trained, the weights of $l$ are fixed. Now consider two functions $h_1, h_2 \in \mathcal{H}$ constructed in  a similar fashion as above. The decoder of $h_1$ has the same weights $W$ and $b^\prime$ as $l$ in layer $i$.  In contrast, the weights of $h_2$ are chosen as $W' \neq W$, $b^\prime$ in layer $i$. This is possible because in $\mathcal{H}$, both $W$ and $W'$ are conditioned on the input $I$ where as in $\mathcal{L}$, $W$ is fixed after training. 

If the cardinality of the preimage of $l$ is bigger than the cardinality of the set of all values of the codeword,  there will be two images $I$ and $I'$ with the same codeword $c(I) = c(I')$ for the LVC architecture and hence the same output. However, as shown above, the HOF regime can be trained the encoder can output two distinct  functions $h_1$ and $h_2$ which can generate different outputs for $I$ and $I'$ without increasing the complexity.
Hence $\mathcal{H}_n$ is strictly larger than $\mathcal{L}_n$.
\end{proof}


Having demonstrated HOF as a generalization of existing contextual mapping methods,
in the next section, we  present a novel application of contextual mapping that leverages the compositionality of the estimated mapping functions to aggregate features of multiple objects or multiple viewpoints of the same object. %Results of a quantitative evaluation of this approach can be found in Figure~\ref{fig:performance_multiview}.

%some (potentially arbitrarily chosen) subset of $\theta$ on a per-sample basis, we might allow our encoder to \textit{learn} which parameters in the decoder $\Dec{}$ should be fixed, and which should vary per-sample. 

% The observation that LVC methods reduce the codeword to an additive bias is formalized in Proposition~\ref{lem:codeword-is-bias}.
% \label{sec:proof}
% \begin{proposition}
% \label{lem:codeword-is-bias}
% If $\Dec{}$ is an MLP with no skip connections computing outputs as $\Dec{}(\vec{x};\vec{z})=\Dec{}(\begin{bmatrix}\vec{z}\\\vec{x}\end{bmatrix})$, $\vec{z}$ acts as a bias $\vec{b}$ to the first layer pre-activations computed independently for each sample.
% \end{proposition}

% Further, we note that if $\vec{b}$ is lower dimensional than $\vec{z}$, there exists infinite $\vec{z}^*$ that satisfy $W^\vec{z}\vec{z}^* = W^\vec{z}\vec{z} + \vec{b}$. Thus, if the latent vector $\vec{z}$ is higher dimensional than the activations in the first layer of $\Dec{}$, we see a degeneracy; the additional expressiveness from the higher dimensional $\vec{z}$ is in some sense wasted.

% The \method{} regime follows as a generalization of LVC contextual mapping methods when $|\vec{b}| < |\theta|$, that is, there are other parameters of the mapping function $\Dec{}$ other than biases in the first layer. We call this assumption that $|\vec{b}| < |\theta|$, where the inequality is strict, our \textbf{non-degeneracy assumption} with respect to the architecture of $\Dec{}$. Given this assumption, we make a final observation about the expressiveness of the \method{} regime in comparison to the LVC regime.

% We consider an encoder network $\Enc$ whose final layer is fully-connected and a fixed mapping network architecture $A_\text{Map}$. We define $\mathcal{H}$ and $\mathcal{L}$ as the spaces of all \FuncName{} parameters for architecture $A_\text{Map}$ that can be estimated from an input image $I$ by the \method{} and LVC regimes, respectively, by $\Enc$. Our claim is stated in Theorem~\ref{thm:codeword-bad}.
% \begin{theorem}
% \label{thm:codeword-bad}
% $\mathcal{L} \subseteq \mathcal{H}$. If the network architecture satisfies our non-degeneracy assumption, $\mathcal{L} \subset \mathcal{H}$.
% \end{theorem}

% \newcommand{\memA}{\gamma}
% \newcommand{\memB}{\beta}
% \begin{proof}
% $\mathcal{L} \subseteq \mathcal{H}$ follows from Proposition~\ref{lem:codeword-is-bias} because \method{} can compute all parameters in $\Dec{}$ given an input $I$ while LVC can only compute the first layer biases. To show that the subset is strict, we define two sets of parameters $\memA$ and $\memB$ in $\mathcal{H}$ such that $\memA = \begin{bmatrix}\vec{b}\\\vec{p}\end{bmatrix}$ and $\memB = \begin{bmatrix}\vec{b}\\\vec{q}\end{bmatrix}$. $|\vec{p}| = |\vec{q}| > 0$ by our non-degeneracy assumption. If $\vec{p} \neq \vec{q}$, $\memA$ and $\memB$ cannot both be in $\mathcal{L}$ because under LVC, parameters in the mapping network other than the first layer bias are fixed.
% \end{proof}
